Deep Learning-Enhanced Robotic Subretinal Injection with Real-Time Retinal Motion Compensation

Subretinal injection is a critical procedure for delivering therapeutic agents to treat retinal diseases such as age-related macular degeneration (AMD). However, retinal motion caused by physiological factors such as respiration and heartbeat significantly impacts precise needle positioning, increasing the risk of retinal pigment epithelium (RPE) damage. This paper presents a fully autonomous robotic subretinal injection system that integrates intraoperative optical coherence tomography (iOCT) imaging and deep learning-based motion prediction to synchronize needle motion with retinal displacement. A Long Short-Term Memory (LSTM) neural network is used to predict internal limiting membrane (ILM) motion, outperforming a Fast Fourier Transform (FFT)-based baseline model. Additionally, a real-time registration framework aligns the needle tip position with the robot's coordinate frame. Then, a dynamic proportional speed control strategy ensures smooth and adaptive needle insertion. Experimental validation in both simulation and ex vivo open-sky porcine eyes demonstrates precise motion synchronization and successful subretinal injections. The experiment achieves a mean tracking error below 16.4 {\mu}m in pre-insertion phases. These results show the potential of AI-driven robotic assistance to improve the safety and accuracy of retinal microsurgery.

==> backup/backup.tex <==
% contains texts that is not used here, but maybe in the future

% Explain the adaptive control (Mojtaba Help)
To precisely align the needle tip with the retina layer, we implemented a control algorithm that leverages segmentation results. Specifically, we utilized the inferred position of the inner limiting membrane (ILM) layer from a neural network-based segmentation model. The choice of the ILM layer over other retinal layers is based on several key factors: 1. Due to the nature of optical coherence tomography (OCT) imaging, light penetration and scattering effects make the ILM the most reliably detected layer. 2. Our task requires synchronized motion between the needle tip and a retinal layer. The ILM, as the topmost layer of the retina, provides optimal visibility for real-time validation. 

Instead of using a constant velocity controller, as proposed by Demir et al. [Reference], which lacks the capability to adapt speed dynamically based on the needle's position relative to the retina, we implemented an adaptive gain control algorithm. 

The control law is formulated as follows:
\begin{equation}
    \dot{x}_{\text{des}} = \alpha \dot{p}_{\text{des}} - K \Delta p
\end{equation}

in which 

\begin{equation}
    \alpha = \dot{\alpha} \Delta t + \alpha
\end{equation}
\begin{equation}
    \dot{\alpha} = -F \dot{p}_{\text{des}} \Delta p
\end{equation}

This approach is adapted from the method introduced by Mojtaba et al. [Reference], with modifications to simplify implementation while maintaining effectiveness. In specific, $\dot{x}_{\text{des}}$ is the final commanded velocity of the needle. $\alpha$ is an adaptive gain that adjusts dynamically. $\dot{p}_{\text{des}}$ represents the desired velocity of the ILM layer. $K$ is a proportional gain. $\Delta p$ is the position error (distance between ILM and needle tip). $F$ is a scaling factor governing the gain update. $\Delta t$ is the sampling time interval.

To ensure safe operation, the final velocity is constrained within a predefined threshold $v_{\max}$:

\begin{equation}
    v = \min(|\dot{x}_{\text{des}}|, v_{\max})
\end{equation}

The adaptive controller above ensures real-time adaptability, by allowing speed modulation based on the dynamic positioning of the ILM layer. It also offers smooth motion control, by reducing abrupt changes in velocity to enhance surgical safety.





%%%How to make a nice table with hierarchical header
\begin{table*}[t!]
\caption{sfuherhgoeihrgoeihroeijrfoeihr. }
\vspace{-8pt}
\label{tab:Precision_table}
\begin{center}
\begin{tabular}{c | c c c c | c c c c}
\hline

 \multicolumn{6}{c}{\centering Artificial vein phantom}
 & \multicolumn{2}{c}{\centering Embryonic chicken veins} \\
 \hline
% \rowcolor{red!10!blue!15}
  \multicolumn{1}{p{1.5cm}}{\centering Filter}
& \multicolumn{1}{p{1.6cm}}{\centering EMA}
& \multicolumn{1}{p{1.6cm}}{\centering AEWMA}
& \multicolumn{1}{p{1.1cm}}{\centering Test}
& \multicolumn{1}{p{1.1cm}}{\centering p-value}
& \multicolumn{1}{p{1.6cm}}{\centering EMA}
& \multicolumn{1}{p{1.6cm}}{\centering AEWMA}
& \multicolumn{1}{p{1.1cm}}{\centering Test}
& \multicolumn{1}{p{1.1cm}}{\centering p-value}
\\

\hline
$\#$ Fertilized eggs & -- & -- & -- & -- & 10 & 10 & -- & -- \\ 
$\#$ Insertions & 30 & 30 & -- & -- & 30 & 30 & -- & -- \\ 
$\#$ TP & 20 & 26 & -- & -- & 13 & 21 & -- & -- \\ 
$\#$ FP & 3 & 1 & -- & -- & 10 & 4 & -- & -- \\ 
$\#$ TN & 0 & 0 & -- & -- & 0 & 0 & -- & -- \\ 
$\#$ FN & 7 & 3 & -- & -- & 7 & 5 & -- & -- \\ 
$\#$ DP & -- & -- & -- & -- & 3 & \textbf{0} & -- & -- \\  
Accuracy (\%) & 66.7 & \textbf{86.6} & Fisher & \textbf{0.047} & 43.33 & \textbf{70.0} & Fisher  & \textbf{0.024}    \\
Precision (\%) & 86.9 & 96.3 & Fisher & 0.2 & 56.52 & \textbf{84.0} & Fisher &  \textbf{0.03}   \\
Recall (\%) & 74.1 & 89.6 & Fisher & 0.09 & 65.0 & 80.76 & Fisher  &   0.13   \\
F1-score (\%) & 80.0 & 92.8 & -- & -- & 63.41 & 82.34 & --& --     \\
Delay (ms) & 45.9$\pm$10.4 & \textbf{3.0$\pm$1.1} & t-test& $<$\textbf{0.01} & 43.7$\pm$13.1 & \textbf{5.3}$\pm$\textbf{1.4} & t-test & $<$\textbf{0.01}    \\
Travel ($\mu$m) & 127.9$\pm$38.6 & \textbf{10.8$\pm$3.8} & t-test& $<$\textbf{0.01}  & 121.9$\pm$54.7 & \textbf{14.9}$\pm$\textbf{5.0} & t-test & $<$\textbf{0.01}    \\


\hline
\end{tabular}
\end{center}
\vspace{-12pt}
\end{table*}

